Tracking Holistic Object Representations

Recent advances in visual tracking are based on siamese feature extractors and template matching. For this category of trackers, latest research focuses on better feature embeddings and similarity measures. In this work, we focus on building holistic object representations for tracking. We propose a framework that is designed to be used on top of previous trackers without any need for further training of the siamese network. The framework leverages the idea of obtaining additional object templates during the tracking process. Since the number of stored templates is limited, our method only keeps the most diverse ones. We achieve this by providing a new diversity measure in the space of siamese features. The obtained representation contains information beyond the ground truth object location provided to the system. It is then useful for tracking itself but also for further tasks which require a visual understanding of objects. Strong empirical results on tracking benchmarks indicate that our method can improve the performance and robustness of the underlying trackers while barely reducing their speed. In addition, our method is able to match current state-of-the-art results, while using a simpler and older network architecture and running three times faster.

==> shortcuts.tex <==
\usepackage{amsmath,amssymb,amsthm}
\usepackage{graphicx}
\usepackage{xspace}
\RequirePackage[dvips]{epsfig} 
\RequirePackage{float}
\RequirePackage{fancyhdr}
\setlength{\headheight}{14.5pt}
\RequirePackage{pstricks,pst-plot,psfrag}
\RequirePackage{multirow}
\RequirePackage{rotating}
\RequirePackage{units}
\usepackage{booktabs}
% \RequirePackage[dvipdfm]{geometry}
\usepackage{pgfplots}
\newlength\figureheight
\newlength\figurewidth
\pgfplotsset{compat=1.14}
\usepackage{caption}
\usepackage{array}
\usepackage{subcaption}
\usepackage{setspace}
\usepackage{enumitem}

\DeclareMathOperator*{\minimize}{minimize}

% %Set up nice tables using the tabular package
% %Make \toprule and \bottomrule thicker than \midrule
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\usepackage{tabularx}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

% %Set up the siunitx package, particularly for using the S column type in tables
\usepackage{etoolbox,siunitx}
\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries

%_______________extra commands_______________%

\newcommand\MyBox[2]{
  \fbox{\lower0.75cm
    \vbox to 1.7cm{\vfil
      \hbox to 1.7cm{\hfil\parbox{1.4cm}{#1}\hfil}
      \vfil}%
  }%
}

\newcommand\MyBoxSmall[2]{
  \fbox{\lower0.0cm
    \vbox to 0.65cm{\vfil
      \hbox to 0.65cm{\hfil\parbox{1.4cm}{#1}\hfil}
      \vfil}%
  }%
}

\newcommand{\axel}[1]{{\color{blue}[Axel: #1]}}
\newcommand{\eli}[1]{{\color{orange}[Eli: #1]}}
\newcommand{\TODO}[1]{{\color{red}[TODO #1]}}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot} \def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot} \def\iid{i.i.d\onedot}
\def\Fig{Fig\onedot} \def\Eqn{Eqn\onedot} \def\Sec{Sec\onedot} \def\Alg{Alg\onedot}
\makeatother
